Beyond 200 Gb/s/lane: An Analytical Approach to Optimal Detection in Shaped IM-DD Optical Links with Relative Intensity Noise

Next-generation intensity-modulation (IM) and direct-detection (DD) systems used in data centers are expected to operate at 400 Gb/s/lane and beyond. Such rates can be achieved by increasing the system bandwidth or the modulation format, which in turn requires maintaining or increasing the signal-to-noise ratio (SNR). Such SNR requirements can be achieved by increasing the transmitted optical power. This increase in optical power causes the emergence of relative intensity noise (RIN), a signal-dependent impairment inherent to the transmitter laser, which ultimately limits the performance of the system. In this paper, we develop an analytical symbol error rate (SER) expression for the optimal detector for the IM-DD optical link under study. The developed expression takes into account the signal-dependent nature of RIN and does not make any assumptions on the geometry or probability distribution of the constellation. Our expression is therefore applicable to general probabilistically and/or geometrically shaped systems. Unlike results available in the literature, our proposed expression provides a perfect match to numerical simulations of probabilistic and geometrically shaped systems.

==> sections/A2.authors.tex <==
\begin{IEEEbiographynophoto}{Felipe Villenas}
was born in Vi\~na del Mar, Chile, in 1998. He received the Electronics Engineer’s degree (Ingeniero Civil Electrónico) and the M.Sc. degree (Magíster en Ciencias de la Ingeniería Electrónica) from Universidad Técnica Federico Santa María, Valparaíso, Chile, in 2021 and 2023, respectively. Since April 2024, he is a PhD student at the ICT Lab in the Signal Processing Systems (SPS) Group, Eindhoven University of Technology (TU/e), the Netherlands.
His research interests are the design of novel digital signal processing schemes and modulation formats for high-speed and short-reach fiber-optic communication systems. 
\end{IEEEbiographynophoto}
\begin{IEEEbiographynophoto}{Kaiquan Wu} was born in Changsha, China, in 1994. He received his B.Sc. and M.Sc. in Communication Engineering from the College of Information Science and Engineering, Hunan University (HNU), China. He was in the state key laboratory of fiber communication during the Master period. He obtained his Ph.D. degree in 2023 from the Eindhoven University of Technology (TU/e), the Netherlands. His main research focuses on designing pragmatic and novel digital signal processing schemes, including error correction code, coded modulation, and channel modeling, for fiber-optic communication systems.
\end{IEEEbiographynophoto}
\begin{IEEEbiographynophoto}{Yunus Can Gültekin}
(S’10) was born in Izmir, Turkey. He received the B.Sc. and M.Sc. degrees in electrical and electronics engineering from Middle East Technical University, Ankara, Turkey, in 2013 and 2015, respectively.  He obtained his Ph.D. degree in 2020 from the Eindhoven University of Technology (TU/e), the Netherlands. During 2020-2023, he held a postdoctoral position at TU/e. Since January 2024, he has been a permanent research staff member at TU/e. His research focuses on understanding the requirements of future wireless/optical communications and quantum key distribution systems, and developing coded modulation and signal processing solutions for these systems using tools from information and communication theory. His research has received multiple awards, including Best Paper awards at the 2018 WIC/IEEE Symposium on Information Theory and Signal Processing in the Benelux and at the 2022 Optica Advanced Photonics Congress, a 2023 Quantum Delta NL exchange visit grant, and a 2024 International Excellence Fellowship from the Karlsruhe Institute of Technology.
\end{IEEEbiographynophoto}
\begin{IEEEbiographynophoto}{Jamal Riani} was born in Tetouan, Morocco, in 1977. He received the degrees in engineering from the Ecole Polytechnique, Palaiseau, France, in 1999, and the Ecole National Supéieure de Télécommunications (ENST), Paris, France, in 2001. He obtained his Ph.D. degree in 2008 from the Eindhoven University of Technology (TU/e), the Netherlands. Since 2007 he has been working as an engineer at Marvell Technology, Inc., in San José, California, USA.
\end{IEEEbiographynophoto}
\begin{IEEEbiographynophoto}{Alex Alvarado}
 (S’06–M’11–SM’15) was born in Quellón, on the island of Chiloé, Chile. He received the Electronics Engineer’s degree (Ingeniero Civil Electrónico) and the M.Sc. degree (Magíster en Ciencias de la Ingeniería Electrónica) from Universidad Técnica Federico Santa María, Valparaíso, Chile, in 2003 and 2005, respectively, and the Licentiate of Engineering degree
(Teknologie Licentiatexamen) and Ph.D. degree from the Chalmers University of Technology, Gothenburg, Sweden, in 2008 and 2011, respectively.
During 2012–2014, he was a Marie Curie Intra-European Fellow with the University of Cambridge, Cambridge, U.K., and during 2011–2012, he was a Newton International Fellow with the same institution. He is currently a Senior Research Associate at the Optical Networks Group, University College London, London, U.K. His general research interests include digital communications, coding, and information theory. In 2008, he received the Merit Scholarship Program for Foreign Students, granted by the Ministere de l’Éducation, du Loisir et du Sports du Québec. He received the 2009 IEEE Information Theory Workshop Best Poster Award, the 2013 IEEE Communication Theory Workshop Best Poster Award, and the 2015 IEEE Transaction on Communications Exemplary
Reviewer Award.
\end{IEEEbiographynophoto}
\vfill
